The Lyman Alpha Reference Sample XV. Relating Ionised Gas Kinematics with Lyman-$\alpha$ observables

Gas kinematics affect the radiative transfer and escape of hydrogen Lyman-$\alpha$ (Ly$\alpha$) emission from galaxies. We investigate this interplay empirically by relating the ionised gas kinematics of 42 galaxies in the extended Ly$\alpha$ Reference Sample with their Ly$\alpha$ escape fractions, $f_\rm{esc}$, Ly$\alpha$ equivalent widths, $\rm{EW}_\rm{Ly\alpha}$, and Ly$\alpha$ luminosities, $L_\rm{Ly\alpha}$. To this aim we use PMAS integral-field spectroscopic observations of the Balmer-$\alpha$ line. We calculate shearing velocities, $v_\rm{shear}$, and intrinsic velocity dispersions, $\sigma_0^\rm{obs}$ (empirically corrected for beam-smearing effects), as global kinematical measures for each galaxy. The sample is characterised by highly turbulent motions and more than half of the sample shows dispersion dominated kinematics. We uncover clear trends between Ly$\alpha$ observables and global kinematical statistics. We discuss statistically the importance of $v_\rm{shear}$, $\sigma_0^\rm{obs}$, and $v_\rm{shear}/\sigma_0^\rm{obs}$ for regulating the Ly$\alpha$ observables in comparison to other galaxy parameters. It emerges that $\sigma_0^\rm{obs}$ is the dominating parameter for $\rm{EW}_\rm{Ly\alpha}$ and that is as important as nebular extinction, gas covering fraction, and ionising photon production efficiency in regulating $f_\rm{esc}$. A simple scenario where the starburst age is simultaneously regulating turbulence, $\rm{EW}_\rm{Ly\alpha}$, and $f_\rm{esc}$ does not find support by our observations. However, we show that the small scale distribution of dust appears to be influenced by turbulence in some galaxies. In support of our observational result we discuss how turbulence is theoretically expected to play a significant role in modulating $f_\rm{esc}$. (abridged)

==> table2_texinclude <==
\begin{tabular}{ccccSrcrSrccr}
\hline \hline \noalign{\smallskip}
ID & kin. & $\cos(i)$ & $(b/a)_\mathrm{I}$ & $\mathrm{EW}_\mathrm{Ly\alpha}$ & $f_\mathrm{esc}^\mathrm{Ly\alpha}$ & Ly$\alpha$/H$\alpha$ & $v_\mathrm{shear}$ & $\sigma_0^\mathrm{obs}$ & $v_\mathrm{shear} / \sigma_0^\mathrm{obs}$ & $\sigma_\mathrm{tot}$ \\
{} & class & {} & {} & \multicolumn{1}{c}{[\AA{}]} & {} & {} & \multicolumn{1}{c}{[km\,s$^{-1}$]} & [km\,s$^{-1}$] & {} & [km\,s$^{-1}$]\\ \hline \noalign{\smallskip}
L01 & PR &  \dots  &  0.42 &  $ 42.2^{+0.4}_{-0.5} $ & $ 0.134 \pm 0.002 $ &$ 1.63^{+0.02}_{-0.02} $ &$ 52.4^{+1.6}_{-2.8} $ & $ 47.2 \pm 0.6 $ &$ 1.11^{+0.04}_{-0.06} $  &  60.5  \\
L02 & CK &  \dots  &  0.40 &  $ 56.7^{+1.3}_{-1.9} $ & $ 0.299 \pm 0.010 $ &$ 2.61^{+0.06}_{-0.08} $ &$ 15.4^{+8.0}_{-2.9} $ & $ 38.2 \pm 0.7 $ &$ 0.40^{+0.21}_{-0.08} $  &  46.0  \\
L03 & PR &  \dots  &  0.54 &  $ 34.2^{+1.3}_{-1.8} $ & $ 0.005 \pm 0.000 $ &$ 0.31^{+0.01}_{-0.02} $ &$ 130.2^{+5.4}_{-6.7} $ & $ 77.3 \pm 2.9 $ &$ 1.68^{+0.10}_{-0.10} $  &  130.9  \\
L04 & CK &  \dots  &  0.38 &  $ 2.1^{+0.5}_{-0.4} $  & $ 0.006 \pm 0.001 $ &$ 0.07^{+0.02}_{-0.02} $ &$ 68.2^{+2.9}_{-5.7} $ & $ 43.0 \pm 0.3 $ &$ 1.58^{+0.07}_{-0.13} $  &  55.1  \\
L05 & PR &  \dots  &  0.43 &  $ 24.9^{+0.5}_{-0.5} $ & $ 0.126 \pm 0.002 $ &$ 1.53^{+0.03}_{-0.03} $ &$ 30.6^{+5.8}_{-1.2} $ & $ 51.2 \pm 0.5 $ &$ 0.60^{+0.11}_{-0.02} $  &  54.7  \\
L06 & CK &  \dots  &  0.49 &  $ \leq 2.4 $ &   $ \leq 0.012 $ &$ \leq 0.14 $ &$ 50.6^{+1.9}_{-1.0} $ & $ 26.2 \pm 0.5 $ &$ 1.94^{+0.08}_{-0.05} $  &  58.9  \\
L07 & PR &  \dots  &  0.47 &  $ 38.8^{+0.9}_{-1.0} $ & $ 0.111 \pm 0.002 $ &$ 1.76^{+0.04}_{-0.04} $ &$ 26.0^{+4.9}_{-2.7} $ & $ 60.6 \pm 0.8 $ &$ 0.43^{+0.08}_{-0.04} $  &  67.4  \\
L08 & RD &  0.63   &  0.71 &  $ 17.3^{+1.3}_{-0.9} $ & $ 0.006 \pm 0.000 $ &$ 0.37^{+0.03}_{-0.02} $ &$ 148.9^{+4.4}_{-3.2} $ & $ 41.2 \pm 0.4 $ &$ 3.61^{+0.11}_{-0.09} $  &  111.8  \\
L09 & CK &  \dots  &  0.26 &  $ 9.8^{+0.5}_{-0.5} $ & $ 0.016 \pm 0.001 $ &$ 0.31^{+0.01}_{-0.01} $ &$ 159.6^{+3.0}_{-8.5} $ & $ 56.1 \pm 0.4 $ &$ 2.84^{+0.06}_{-0.15} $  &  112.7  \\
L10 & PR &  \dots  &  0.49 &  $ \leq 2.1 $ & $ \leq 0.003 $ &$ \leq 0.12 $ &$ 32.4^{+5.5}_{-6.0} $ & $ 36.5 \pm 0.6 $ &$ 0.89^{+0.15}_{-0.16} $  &  49.2  \\
L11 & RD &  0.00   &  0.34 &  $ 20.5^{+1.0}_{-0.7} $ & $ 0.065 \pm 0.009 $ &$ 1.81^{+0.13}_{-0.10} $ &$ 149.1^{+11.2}_{-6.1} $ & $ 60.9 \pm 1.4 $ &$ 2.45^{+0.19}_{-0.12} $  &  114.8  \\
L12 & CK &  \dots  &  0.69 &  $ 18.1^{+1.0}_{-1.0} $ & $ 0.027 \pm 0.001 $ &$ 1.11^{+0.07}_{-0.06} $ &$ 81.3^{+18.7}_{-3.3} $ & $ 64.8 \pm 1.1 $ &$ 1.26^{+0.29}_{-0.06} $  &  81.3  \\
L13 & CK &  \dots  &  0.50 &  $ \leq 1.8 $ & $ \leq 0.004 $ &$ \leq 0.14 $ &$ 168.5^{+18.7}_{-3.3} $ & $ 61.0 \pm 0.9 $ &$ 2.77^{+0.31}_{-0.07} $  &  97.3  \\
L14 & CK &  \dots  &  0.89 &  $ 49.0^{+2.3}_{-2.1} $ & $ 0.263 \pm 0.010 $ &$ 2.94^{+0.11}_{-0.11} $ &$ 38.8^{+2.3}_{-0.1} $ & $ 59.0 \pm 1.2 $ &$ 0.66^{+0.04}_{-0.02} $  &  72.9  \\
E01 & CK &  \dots  &  0.88 &  $ 21.2^{+0.3}_{-0.3} $ & $ 0.012 \pm 0.000 $ &$ 0.39^{+0.00}_{-0.00} $ &$ 43.0^{+2.1}_{-2.0} $ & $ 55.6 \pm 0.3 $ &$ 0.77^{+0.04}_{-0.04} $  &  58.7  \\
E02 & PR &  \dots  &  0.78 &  $ 12.4^{+0.5}_{-0.3} $ & $ 0.061 \pm 0.002 $ &$ 0.54^{+0.02}_{-0.01} $ &$ 17.7^{+2.1}_{-0.3} $ & $ 31.2 \pm 0.4 $ &$ 0.57^{+0.07}_{-0.01} $  &  45.2  \\
E03 & PR &  \dots  &  0.49 &  $ 4.4^{+0.5}_{-0.4} $ & $ 0.005 \pm 0.001 $ &$ 0.12^{+0.01}_{-0.01} $ &$ 181.8^{+1.1}_{-2.8} $ & $ 40.7 \pm 0.2 $ &$ 4.46^{+0.04}_{-0.07} $  &  129.0  \\
E04 & RD &  0.91   &  0.45 &  $ 17.1^{+0.5}_{-0.4} $ & $ 0.070 \pm 0.002 $ &$ 1.05^{+0.03}_{-0.03} $ &$ 60.7^{+2.4}_{-1.7} $ & $ 43.7 \pm 0.4 $ &$ 1.39^{+0.06}_{-0.04} $  &  66.7  \\
E05 & RD &  \dots  &  0.66 &  $ 26.5^{+1.0}_{-0.9} $ & $ 0.148 \pm 0.006 $ &$ 1.60^{+0.06}_{-0.05} $ &$ 145.9^{+1.9}_{-1.3} $ & $ 37.7 \pm 0.3 $ &$ 3.88^{+0.06}_{-0.05} $  &  121.2  \\
E06 & RD &  0.74   &  0.67 &  $ 12.6^{+1.4}_{-1.0} $ & $ 0.060 \pm 0.005 $ &$ 0.99^{+0.11}_{-0.07} $ &$ 61.3^{+1.2}_{-1.7} $ & $ 28.7 \pm 0.2 $ &$ 2.14^{+0.05}_{-0.06} $  &  59.5  \\
E07 & CK &  \dots  &  0.42 &  $ 7.1^{+1.1}_{-1.4} $ & $ 0.032 \pm 0.006 $ &$ 0.32^{+0.05}_{-0.06} $ &$ 93.1^{+1.6}_{-19.3} $ & $ 30.6 \pm 0.5 $ &$ 3.03^{+0.07}_{-0.63} $  &  71.7  \\
E08 & RD &  0.83   &  0.74 &  $ 16.7^{+1.4}_{-1.4} $ & $ 0.017 \pm 0.002 $ &$ 0.79^{+0.07}_{-0.07} $ &$ 88.0^{+1.6}_{-3.3} $ & $ 25.4 \pm 0.3 $ &$ 3.46^{+0.08}_{-0.14} $  &  64.3  \\
E09 & PR &  \dots  &  0.67 &  $ 5.6^{+1.0}_{-1.0} $ & $ 0.054 \pm 0.010 $ &$ 0.61^{+0.11}_{-0.11} $ &$ 31.9^{+6.2}_{-4.4} $ & $ 32.8 \pm 0.7 $ &$ 0.97^{+0.19}_{-0.14} $  &  47.4  \\
E10 & RD &  0.39   &  0.24 &  $ 16.8^{+2.4}_{-1.9} $ & $ 0.016 \pm 0.002 $ &$ 0.67^{+0.09}_{-0.08} $ &$ 121.6^{+2.2}_{-2.2} $ & $ 43.7 \pm 0.4 $ &$ 2.78^{+0.06}_{-0.06} $  &  94.4  \\
E11 & RD &  0.85   &  0.72 &  $ 8.9^{+1.0}_{-0.9} $ & $ 0.065 \pm 0.007 $ &$ 0.68^{+0.08}_{-0.07} $ &$ 77.4^{+1.3}_{-2.1} $ & $ 46.7 \pm 0.4 $ &$ 1.66^{+0.03}_{-0.05} $  &  65.8  \\
E12 & RD &  0.41   &  0.38 &  $ \leq 1.3 $ & $ \leq 0.002 $ &$ \leq 0.04 $ &$ 126.4^{+1.7}_{-1.5} $ & $ 35.4 \pm 0.3 $ &$ 3.57^{+0.06}_{-0.05} $  &  93.5  \\
E13 & CK &  \dots  &  0.81 &  $ 37.7^{+1.6}_{-1.4} $ & $ 0.207 \pm 0.008 $ &$ 2.86^{+0.11}_{-0.10} $ &$ 21.7^{+3.3}_{-2.2} $ & $ 61.7 \pm 1.3 $ &$ 0.35^{+0.05}_{-0.04} $  &  55.7  \\
E14 & RD &  0.91   &  0.93 &  $ \leq 1.3 $ & $ \leq 0.005 $ &$ \leq 0.06 $ &$ 55.2^{+1.5}_{-2.5} $ & $ 31.9 \pm 0.7 $ &$ 1.73^{+0.06}_{-0.09} $  &  54.1  \\
E15 & PR &  \dots  &  0.60 &  $ 20.0^{+3.0}_{-2.6} $ & $ 0.124 \pm 0.018 $ &$ 1.25^{+0.18}_{-0.16} $ &$ 50.4^{+4.5}_{-3.2} $ & $ 31.1 \pm 0.4 $ &$ 1.62^{+0.15}_{-0.11} $  &  47.4  \\
E16 & RD &  0.39   &  0.48 &  $ \leq 2.4 $ & $ \leq 0.009 $ &$ \leq 0.18 $ &$ 76.9^{+4.3}_{-1.6} $ & $ 23.9 \pm 0.4 $ &$ 3.22^{+0.19}_{-0.09} $  &  59.7  \\
E17 & RD &  0.64   &  0.39 &  $ 19.4^{+3.1}_{-2.5} $ & $ 0.082 \pm 0.012 $ &$ 1.36^{+0.21}_{-0.17} $ &$ 85.3^{+1.8}_{-5.0} $ & $ 24.7 \pm 0.6 $ &$ 3.43^{+0.12}_{-0.22} $  &  72.8  \\
E18 & RD &  0.08   &  0.26 &  $ 7.9^{+2.7}_{-3.3} $ & $ 0.030 \pm 0.013 $ &$ 0.50^{+0.17}_{-0.22} $ &$ 74.9^{+2.2}_{-3.5} $ & $ 26.4 \pm 0.6 $ &$ 2.84^{+0.11}_{-0.14} $  &  63.9  \\
E19 & RD &  0.78   &  0.47 &  $ 10.0^{+2.0}_{-1.6} $ & $ 0.064 \pm 0.010 $ &$ 0.63^{+0.12}_{-0.10} $ &$ 52.0^{+6.4}_{-1.6} $ & $ 28.2 \pm 0.6 $ &$ 1.85^{+0.23}_{-0.07} $  &  50.4  \\
E20 & PR &  \dots  &  0.91 &  $ 7.9^{+1.8}_{-2.0} $ & $ 0.031 \pm 0.008 $ &$ 0.41^{+0.10}_{-0.10} $ &$ 37.1^{+1.2}_{-1.8} $ & $ 36.9 \pm 0.5 $ &$ 1.00^{+0.04}_{-0.05} $  &  45.4  \\
E21 & RD &  0.37   &  0.28 &  $ 9.0^{+3.5}_{-3.1} $ & $ 0.047 \pm 0.033 $ &$ 0.94^{+0.37}_{-0.33} $ &$ 50.6^{+7.1}_{-3.6} $ & $ 26.6 \pm 0.8 $ &$ 1.90^{+0.27}_{-0.15} $  &  57.7  \\
E22 & CK &  \dots  &  0.45 &  $ 6.8^{+0.5}_{-0.6} $ & $ 0.056 \pm 0.005 $ &$ 0.51^{+0.04}_{-0.04} $ &$ 38.6^{+18.3}_{-3.0} $ & $ 39.5 \pm 1.3 $ &$ 0.98^{+0.47}_{-0.08} $  &  55.5  \\
E23 & PR &  \dots  &  0.81 &  $ 6.5^{+1.0}_{-1.1} $ & $ 0.040 \pm 0.007 $ &$ 0.35^{+0.05}_{-0.06} $ &$ 31.6^{+6.2}_{-2.7} $ & $ 23.9 \pm 0.7 $ &$ 1.32^{+0.26}_{-0.12} $  &  49.6  \\
E24 & RD &  0.95   &  0.88 &  $ 22.3^{+1.0}_{-0.9} $ & $ 0.004 \pm 0.000 $ &$ 0.64^{+0.03}_{-0.03} $ &$ 95.0^{+8.2}_{-2.8} $ & $ 78.0 \pm 2.9 $ &$ 1.23^{+0.12}_{-0.06} $  &  94.8  \\
E25 & PR &  \dots  &  0.71 &  $ 9.6^{+1.1}_{-1.2} $ & $ 0.094 \pm 0.012 $ &$ 0.84^{+0.10}_{-0.11} $ &$ 48.9^{+3.1}_{-5.7} $ & $ 34.1 \pm 0.5 $ &$ 1.43^{+0.09}_{-0.17} $  &  45.0  \\
E26 & RD &  \dots  &  0.43 &  $ 21.5^{+1.7}_{-1.8} $ & $ 0.059 \pm 0.005 $ &$ 0.68^{+0.05}_{-0.05} $ &$ 89.0^{+0.8}_{-2.3} $ & $ 30.9 \pm 0.7 $ &$ 2.86^{+0.08}_{-0.10} $  &  65.6  \\
E27 & RD &  0.95   &  0.73 &  $ 18.8^{+1.6}_{-1.5} $ & $ 0.115 \pm 0.011 $ &$ 1.10^{+0.09}_{-0.09} $ &$ 48.9^{+0.7}_{-1.8} $ & $ 26.6 \pm 0.6 $ &$ 1.83^{+0.05}_{-0.08} $  &  58.9  \\
E28 & PR &  \dots  &  0.81 &  $ 3.1^{+1.3}_{-1.1} $ & $ 0.013 \pm 0.005 $ &$ 0.16^{+0.06}_{-0.06} $ &$ 14.7^{+0.9}_{-2.4} $ & $ 25.8 \pm 0.5 $ &$ 0.57^{+0.04}_{-0.09} $  &  33.5  \\
\hline \hline
\end{tabular}


